Finite-gap CMV matrices: Periodic coordinates and a Magic Formula

We prove a bijective unitary correspondence between 1) the isospectral torus of almost-periodic, absolutely continuous CMV matrices having fixed finite-gap spectrum and 2) special periodic block-CMV matrices satisfying a Magic Formula. This latter class arises as spectrally-dependent operator M\"obius transforms of certain generating CMV matrices which are periodic up to a rotational phase; for this reason we call them "MCMV". Such matrices are related to a choice of orthogonal rational functions on the unit circle, and their correspondence to the isospectral torus follows from a functional model in analog to that of GMP matrices. As a corollary of our construction we resolve a conjecture of Simon; namely, that Caratheodory functions associated to such CMV matrices arise as quadratic irrationalities.

==> header.tex <==
% #########################################################
% ### P A C K A G E S #####################################
% #########################################################
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[ngerman,english]{babel}
\usepackage{lmodern}



\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amscd}
\usepackage{amsbsy}

\usepackage{pdfpages}
\usepackage{fancyhdr}
\usepackage{geometry}
\usepackage{setspace}
\usepackage{xcolor}
%\usepackage{tocloft}
\usepackage{pifont}

\usepackage{graphicx}
\usepackage{tabularx}
\usepackage{epsfig}
\usepackage[all]{xy}
\usepackage{tikz}
\usetikzlibrary{matrix}

\usepackage{fixmath}

\usepackage{appendix}



%\usepackage{eurosym}
\usepackage{enumerate}



\usepackage[sort, numbers]{natbib}
\usepackage{bibentry}
% hyperref should be the last package included
%\usepackage[colorlinks,citecolor=red,linkcolor=blue]{hyperref}


% #########################################################
% ### E N V I R O N M E N T S #############################
% #########################################################
\newtheorem{theorem}{Theorem}[section]


\newtheorem{theoremm}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{question}[theorem]{Question}
\newtheorem*{remark}{Remark}
\newtheorem*{remarks}{Remarks}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{example}[theorem]{Example}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\numberwithin{equation}{section}

% #########################################################
% ### C O M M A N D S #####################################
% #########################################################
\newcommand{\N}{{\mathbb N}}
\newcommand{\Z}{{\mathbb Z}}
\renewcommand{\P}{{\mathbb P}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\D}{{\mathbb D}}
\newcommand{\T}{{\mathbb T}}
\newcommand{\A}{{\mathbb A}}
\newcommand{\bbH}{{\mathbb H}}
\newcommand{\E}{{\mathsf E}}
\newcommand{\V}{{\mathbb V}}
\newcommand{\mj}{j}
\newcommand{\mjH}{j}

\newcommand{\cov}{{\operatorname{cov}}}
\newcommand{\supp}{{\operatorname{supp}}}
\newcommand{\Res}{\operatorname{Res}}
\newcommand{\GMP}{\text{\rm GMP}}
\newcommand{\oc}{\overset{\circ}}
\newcommand{\err}{{\mathrm{err}}}
\newcommand{\disc}{{\mathrm{disc}}}
\newcommand{\simu}{{\mathrm{sim}}}
\newcommand{\QMC}{{\mathrm{QMC}}}
\newcommand{\MC}{{\mathrm{MC}}}
\newcommand{\her}{{\mathrm{her}}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\lin}{\mathrm{span}}
\newcommand{\integ}{\mathrm{int}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\clos}{\text{\rm clos}\,}
\newcommand{\diag}{\operatorname{diag}}

\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{M}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cM}{{T}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cZ}{{\mathcal{Z}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cU}{{U}}
\newcommand{\cv}{{\mathcal{v}}}




\newcommand{\fA}{{\mathfrak{A}}}
\newcommand{\fB}{{\mathfrak{B}}}
\newcommand{\fH}{{\mathfrak{H}}}
\newcommand{\fK}{{\mathfrak{K}}}
\newcommand{\fP}{{\mathfrak{P}}}
\newcommand{\fX}{{\mathfrak{X}}}
\newcommand{\fS}{{\mathfrak{S}}}
\newcommand{\fa}{{\mathfrak{a}}}
\newcommand{\fb}{{\mathfrak{b}}}
\newcommand{\fe}{{\mathfrak{e}}}
\newcommand{\ff}{{\mathfrak{f}}}
\newcommand{\fj}{{\mathfrak{j}}}
\newcommand{\fm}{{\mathfrak{m}}}
\newcommand{\fp}{{\mathfrak{p}}}
\newcommand{\fu}{{\mathfrak{u}}}
\newcommand{\fv}{{\mathfrak{v}}}
\newcommand{\fw}{{\mathfrak{w}}}
\newcommand{\fz}{{\mathfrak{z}}}
\newcommand{\fx}{{\mathfrak{x}}}



\newcommand{\bb}{\mathbf{b}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bp}{{\mathbf{p}}}
\newcommand{\bR}{{\mathbf{R}}}
\newcommand{\gammab}{{\boldsymbol{\gamma}}}
\newcommand{\balpha}{{\boldsymbol{\alpha}}}
\newcommand{\bomega}{{\boldsymbol{\omega}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\bepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\bzeta}{{\boldsymbol{\zeta}}}

\newcommand{\G}{{\Gamma}}
\newcommand{\e}{{\varepsilon}}
\renewcommand{\k}{\varkappa}
\newcommand{\vt}{\vartheta}
\newcommand{\vpi}{\varpi}
\newcommand{\om}{{\omega}}
\newcommand{\z}{\zeta}
\newcommand{\g}{\gamma}
\newcommand{\Up}{\Upsilon}
\renewcommand{\l}{\lambda}
\renewcommand{\a}{\alpha}
\newcommand{\x}{y}
\renewcommand{\chi}{y}
\renewcommand{\b}{\beta}
\renewcommand{\d}{\delta}
\renewcommand{\t}{{\theta}}
\renewcommand{\L}{{\Lambda}}



\newcommand{\dd}{\mathrm{d}}
\newcommand{\spa}{\operatorname{span}}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\renewcommand{\Cap}{\operatorname{Cap}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\dx}{\mathrm{d}x}
\newcommand{\pd}{{\partial}}
\newcommand{\rz}{z^*}

\newcommand{\gdw}{\Leftrightarrow}

\newcommand{\ld}{\operatorname{ld}}

\newcommand{\zu}{z_{\zeta_0}}
\newcommand{\zub}{\overline z_{\zeta_0}}
\newcommand{\zi}{z_{\infty}}
\newcommand{\tzi}{\tilde z_{\infty}}
\newcommand{\ko}{\kappa_0}
\newcommand{\za}{z_\alpha}
\newcommand{\cza}{\overline z_\alpha}

\newcommand{\gO}{g_\Omega}

\newcommand{\vp}{{\vec{p}}}
\newcommand{\vq}{{\vec{q}}}
\newcommand{\vbp}{{\vec{\mathbf{p}}}}
\newcommand{\vd}{{\vec{\delta}_g}}
\renewcommand{\i}{\infty}
%\renewcommand{\vec}{\hspace{-0.1cm}\vec}
\newcommand{\vz}{\vec{\vspace{1cm}z}}


\newcommand{\minus}{\scalebox{0.5}[1.0]{\( -\)}\hspace{-0.04cm}}

 \newcommand{\TODO}[1]{\noindent{\bf \color{cyan}TODO: }{\color{cyan} #1}}

% #########################################################
% ### S T Y L E ###########################################
% #########################################################

\newcommand{\apa}{\mathbf a}
\newcommand{\apr}{\mathbold\rho}
\newcommand{\apC}{\mathcal C}

\newcommand{\mv}{\text{\rm{CMV}}}
\newcommand{\MV}{\text{\rm{MCMV}}}
\newcommand{\per}{\text{\rm{per}}}
\newcommand{\ess}{\text{\rm{ess}}}

\newcommand{\DD}{D_{0}}

